AlphaDPO: Adaptive Reward Margin for Direct Preference Optimization

Aligning large language models (LLMs) with human values and intentions is crucial for their utility, honesty, and safety. Reinforcement learning from human feedback (RLHF) is a popular approach to achieve this alignment, but it faces challenges in computational efficiency and training stability. Recent methods like Direct Preference Optimization (DPO) and Simple Preference Optimization (SimPO) have proposed offline alternatives to RLHF, simplifying the process by reparameterizing the reward function. However, DPO depends on a potentially suboptimal reference model, and SimPO's assumption of a fixed target reward margin may lead to suboptimal decisions in diverse data settings. In this work, we propose $\alpha$-DPO, an adaptive preference optimization algorithm designed to address these limitations by introducing a dynamic reward margin. Specifically, $\alpha$-DPO employs an adaptive preference distribution, balancing the policy model and the reference model to achieve personalized reward margins. We provide theoretical guarantees for $\alpha$-DPO, demonstrating its effectiveness as a surrogate optimization objective and its ability to balance alignment and diversity through KL divergence control. Empirical evaluations on AlpacaEval 2 and Arena-Hard show that $\alpha$-DPO consistently outperforms DPO and SimPO across various model settings, establishing it as a robust approach for fine-tuning LLMs. Our method achieves significant improvements in win rates, highlighting its potential as a powerful tool for LLM alignment. The code is available at https://github.com/junkangwu/alpha-DPO

==> Tables/leadboard.tex <==
% \documentclass{article}
\begin{wraptable}[13]{r}{7.7cm}
    \setlength{\tabcolsep}{1pt}
    \vspace{-1.3em}
    \caption{
    Length-controlled (LC) and raw win rate (WR), and generation lengths of top models on the AlpacaEval 2 Leaderboard. \textbf{\small Bold} are the models we trained. 
    }
    \vspace{-0.2em}
    \centering
        \small
        \resizebox{7.7cm}{!}{\begin{tabular}{l*{3}{c}}
    \toprule
    \multirow{1}{*}{\textbf{Model}} &  {\bf LC (\%)} & {\bf WR (\%)} & \textbf{ Len.} \\
    \midrule
    \rowcolor{lightblue}\textbf{Llama3-Instruct-8B-Ours-v0.2} & 58.5 & 50.4 & 1746 \\
    GPT-4 Turbo (04/09) & 55.0 & 46.1 & 1802  \\ 
    \textbf{Llama3-Instruct-8B-\method-v0.2} & 53.7 & 47.5 & 1777 \\
    GPT-4 Turbo (11/06) & 50.0 & 50.0 & 2049 \\ 
    \textbf{Llama3-Instruct-8B-\method} & 44.7 & 40.5 & 1825 \\
    Claude 3 Opus & 40.5 & 29.1 & 1388 \\
    \textbf{Llama3-Instruct-8B-DPO} & 40.3 & 37.9 & 1837 \\
    % GPT-4 (03/14) & 35.3 & 22.1 & 1371 \\
    Llama3-Instruct-70B & 34.4 & 33.2 & 1919 \\
    % Mistral Large & 32.7 & 21.4 & 1362 \\
    % Mixtral-8x22B-Instruct & 30.9 & 22.2 & 1445  \\
    % Claude 2 & 28.2 & 17.2  \\
    Llama3-Instruct-8B & 26.0 & 25.3 & 1899 \\
    % Gemini 1.0 Pro & 24.4 & 18.2 & 1456 \\
    % Mixtral-8x7B-Instruct & 23.7 & 18.3 \\
    GPT-3.5 Turbo (06/13) & 22.7 & 14.1 & 1328 \\
    \bottomrule
    \end{tabular}}
    \label{tab:leaderboard}
    \end{wraptable}
    
    \setlength{\tabcolsep}{6pt}
    

==> sections/rebuttal.tex <==
\newpage
% \noindent\hrulefill\ \textbf{Summary of Updates}\ \hrulefill
% We have made substantial revisions to the paper based on the comments provided by the meta-reviewer and three reviewers. The major changes are as follows:
\section{Rebuttal}
\subsection{Reviewer 5mgV}

\paragraph{Q1: However, as uniform policy assigns equal probabilities to all responses, this directly implies $\gamma=0$.}

\paragraph{A1:} There seems to be a misunderstanding here, which we would like to clarify. The distributions of the positive and negative samples are not equal. Let's revisit the acquisition method for these samples (e.g., using \texttt{princeton-nlp/llama3-ultrafeedback} dataset):
For each prompt $x$, we generate 5 responses using the SFT model with a sampling temperature of 0.8. We then score these responses with \texttt{llm-blender/PairRM} and select the highest-scoring one as $y_w$ and the lowest-scoring one as $y_l$. 

For the highest-scoring sample $y_w$, it follows a new conditional distribution:
\[
\pi(y \mid x, \text{score}(y) = \max\{\text{score}(y_1), \ldots, \text{score}(y_5)\})
\]
For the lowest-scoring sample $y_l$, it follows:
\[
\pi(y \mid x, \text{score}(y) = \min\{\text{score}(y_1), \ldots, \text{score}(y_5)\})
\]
Each response is generated from the same conditional distribution $\pi_{\text{SFT}}$, implying the same distribution during generation. However, by scoring and selecting using \texttt{llm-blender/PairRM}, there is an inherent selection bias. Thus, the statement "uniform policy assigns equal probabilities to all responses" is inaccurate.

\paragraph{Q2: They claim that when is 0, they get back the SimPO loss.}

\paragraph{A2:} Similarly to \textbf{A1}, the uniform distribution can mitigate the unreliability of $\pi_{\text{ref}}$, but it still lacks sample personalization and remains suboptimal. Our AlphaDPO objective is designed to incorporate the strengths of both DPO and SimPO.

\paragraph{Q3: Their proposed loss in Eqn.12 combines SimPO and DPO loss with an extra stop gradient on the DPO loss.}

\paragraph{A3:} Indeed, from a formal perspective, the AlphaDPO appears as DPO with an additional stop gradient on the Margin term. However, this result demonstrates that SimPO with an offset ($r(x,y_w)-r(x,y_l)-M$) can further enhance performance, presenting theoretical benefits (\textit{c.f.} Section 4) and relationships that, although concise, are effective.

\paragraph{Q4: They introduce an importance sampling correction term for the online SimPO loss. How is that relevant to Lemma 4.2 or any other part of the paper?}

\paragraph{A4:} Online preference optimization, particularly methods like online AI feedback (OAIF) [1] and self-play [2][3], enhances model alignment by generating new data during training. This success has become widely acknowledged in the research community. Therefore, we propose that establishing theoretical consistency with online preference optimization can potentially enhance the performance of offline algorithms.

The underlying logic here is first to define the expression for online SimPO, which is characterized by the continuous updating of sampled data during training. In this process, the data transitions from the offline set $(y_w, y_l) \in D$ to the online set $(y_w, y_l) \in \pi_\theta$. This operation can be viewed as a form of importance sampling. Interestingly, this key technique of importance sampling aligns with the optimization direction of AlphaDPO loss, with both approaches converging in the scenario where $\alpha \to 0$. Consequently, Lemma 4.2 aims to establish a connection between AlphaDPO and the Online SimPO loss, thereby facilitating the integration of these concepts.

[1] Guo et al. Direct Language Model Alignment from Online AI Feedback. CoRR abs/2402.04792 (2024)

[2] Chen et al. Self-Play Fine-Tuning Converts Weak Language Models to Strong Language Models. ICML 2024.

[3] Wu et al. Self-Play Preference Optimization for Language Model Alignment. CoRR abs/2405.00675 (2024)

\paragraph{Q5: I am not sure how Lemma 4.3 contributes. Further, their claim that they improve upon token-level DPO is not correct.}

\paragraph{A5:} There seems to be a misconception that needs clarification. The core contribution of token-level DPO is the introduction of the form $r(x,y_w)-r(x,y_l)-\delta$, similar to DPO with an offset, enabling control over KL divergence. The AlphaDPO follows the form SimPO with an offset $r(x,y_w)-r(x,y_l)-M$, providing performance enhancement and showing that $M$ is more effective than $\delta$. Appendix Table 6 supports this with performance comparisons between TDPO and AlphaDPO. 
These findings illustrate:
\begin{enumerate}
    \item Adding an offset to DPO and its variants is a successful strategy, applicable to both token-level DPO and AlphaDPO.
    \item The choice of offset is still undecided. Under the premise of an unreliable reference model in the SimPO concept, $M$ outperforms $\delta$, offering valuable insights.
\end{enumerate}

\subsection{Reviewer Jeuw}

Certainly! Below are your questions and answers formatted in LaTeX:

---

**Q1: My major concern is that the motivation of the proposed reference policy Eq.(8) is not so clear.**

> **A1:** Firstly, from the perspective of utility theory, the proposed reference policy \(\hat{\pi}_{\text{ref}}(y|x)\) can be understood as follows: the uniform distribution \(U(y|x)\) serves as a baseline, while the term \(\left(\frac{\pi_\theta(y|x)}{\pi_{\text{ref}}(y|x)}\right)^\alpha\) dynamically adjusts the reward margin by balancing the policy and reference models. This design aligns with the concept of relative attractiveness in utility theory, enabling instance-specific reward adaptation.

> Secondly, from a gradient perspective, \(\hat{\pi}_{\text{ref}}(y|x)\) mitigates label flipping issues found in DPO or SimPO. As per the gradient expression in the SimPO framework:

> \[
\nabla_\theta\mathcal{L}_{\mathrm{SimPO}}(\pi_\theta) = -\beta\mathbb{E}_{(x,y_w,y_l)\sim\mathcal{D}}\left[s_\theta\left(\underbrace{\frac{1}{|y_w|}\nabla_\theta\log\pi_\theta(y_w|x)}_{\text{increase likelihood on }y_w} - \underbrace{\frac{1}{|y_l|}\nabla_\theta\log\pi_\theta(y_l|x)}_{\text{decrease likelihood on }y_l}\right)\right]
\]

> where:
\(s_\theta = \sigma\left(\frac{\beta}{|y_l|}\log\pi_\theta(y_l|x) - \frac{\beta}{|y_w|}\log\pi_\theta(y_w|x) + \gamma\right)\).
This can result in a higher weight when the reward estimate is incorrect. Under \(\alpha\)-DPO, we have:
\(s_\theta = \sigma\left(\frac{\beta}{|y_l|}\log\pi_\theta(y_l|x) - \frac{\beta}{|y_w|}\log\pi_\theta(y_w|x) + \gamma + \alpha M(x,y_w,y_l)\right)\),
which increases weight when the reward estimate is accurate through \(M(x,y_w,y_l)\).

> Lastly, the core motivation is to address the unreliability of the existing reference policy, as discussed in Section 3.1. By integrating the policy model, we aim to enhance the reference model's quality, thereby improving model fine-tuning performance. Similar ideas have been presented in recent works \cite{Gorbatovski2024, Liu2024}, which suggest updating the reference model through the policy model:

> \begin{itemize}
> \item \text{Gorbatovski et al. 2024. Learn your reference model for real good alignment. arXiv preprint arXiv:2404.09656}
> \item \text{Liu et al. 2024. Understanding Reference Policies in Direct Preference Optimization. arXiv preprint arXiv:2407.13709}
> \end{itemize}

**Q2: The authors use the Taylor expansion w.r.t \(\log(A-\alpha B)\) on \(\alpha=0\). This makes the lower bound only established around zero, which limits the theoretical contribution.**

> **A2:** We apologize for the error in the initial proof presentation. The correct expression is:

> By expanding \(\log\sigma(A-\alpha B)\) around \(A\) using the first-order Taylor expansion, we obtain: ...

> According to Taylor's theorem: \(f(x) \approx f(a) + f'(a)(x-a)\) and \((\log\sigma(x))' = 1 - \sigma(x)\).
Thus:

> \[
\log\sigma(A-\alpha B) \approx \log\sigma(A) + (\log\sigma(A))^{'}(-\alpha B) = \log\sigma(A) - \alpha B (1 - \sigma(A))
\]

> Given this, the expansion is mathematically valid and not specifically targeting \(\alpha=0\).

**Q3: Moreover, in lines 913 and 914, the authors state that "under the assumption that the reference policy has large errors", but it seems that I do not find it in the lemma, the authors mention it directly in the lemma and discuss why this assumption is mild.**

> **A3:** Thank you for your suggestion. We will make this part of the presentation more precise. The statement "under the assumption that the reference policy has large errors" is indeed the motivation for proposing \(\alpha\)-DPO. As described in Section 3.1, the DPO uses a reference policy that is unreliable. We have revised the manuscript to reflect this clarification.

---

Note: Citations \cite{Gorbatovski2024, Liu2024} in \(\LaTeX\) format refer to the referenced papers. Please update your bibliography accordingly to reflect the details of these papers as per your manuscript.
